PEGASUS: Pre-training with Extracted Gap-sentences for Abstractive Summarization

Recent work pre-training Transformers with self-supervised objectives on large text corpora has shown great success when fine-tuned on downstream NLP tasks including text summarization. However, pre-training objectives tailored for abstractive text summarization have not been explored. Furthermore there is a lack of systematic evaluation across diverse domains. In this work, we propose pre-training large Transformer-based encoder-decoder models on massive text corpora with a new self-supervised objective. In PEGASUS, important sentences are removed/masked from an input document and are generated together as one output sequence from the remaining sentences, similar to an extractive summary. We evaluated our best PEGASUS model on 12 downstream summarization tasks spanning news, science, stories, instructions, emails, patents, and legislative bills. Experiments demonstrate it achieves state-of-the-art performance on all 12 downstream datasets measured by ROUGE scores. Our model also shows surprising performance on low-resource summarization, surpassing previous state-of-the-art results on 6 datasets with only 1000 examples. Finally we validated our results using human evaluation and show that our model summaries achieve human performance on multiple datasets.

==> tables/qualitative.tex <==
\begin{table*}[bth!]
\scriptsize
  \centering
  \renewcommand{\arraystretch}{1.3}
  \begin{tabular}{c|p{0.85\textwidth}}
  \hline
  
  \multicolumn{2}{c}{XSum} \\ \hline
  \makecell{Document\\(ID \#501)} & LMargarita Louis-Dreyfus, Marseille's billionaire owner, said in April that she would sell the club following poor results and protests from fans. McCourt, speaking at a news conference, said: ``I'm very excited about making Marseille a champion again.'' A deal is set to be completed by the end of the year and no fee has yet been disclosed. Appearing alongside Louis-Dreyfus and Marseille mayor Jean-Claude Gaudin, 63-year-old McCourt said he wants a team that can compete ``year in, year out'' to win Ligue 1. Marseille, who finished 13th in 2015/16 and lost to PSG in the French cup final, are 11th after three games this season. \\ \hline
  Summary & Frank McCourt, the former owner of the LA Dodgers baseball team, is set to buy French Ligue 1 club Marseille.  \\ \hline
  Ours & American businessman Frank McCourt has agreed to buy French club Marseille. \\ \hline
  \makecell{Document\\(ID \#4517)} & Miller served his ban from 2004 to 2006 after admitting using blood-boosting agent EPO early in his career. The 39-year-old returned to the sport and has volunteered to educate Britain's young riders. Technical director Shane Sutton said ``nurturing an anti-doping culture'' was at the heart of British Cycling. Millar won stages in road cycling's three most prestigious stage races - the Tour de France, Vuelta a Espana and Giro d'Italia - and also won 2010 Commonwealth gold for Scotland in the road race time trial. The Scot, who retired in 2014, is regarded as one of the sport's leading anti-doping campaigners. Sutton added: ``Having someone of David's calibre on board to support us in this education process is invaluable. He is readily available to share his well-rounded experiences as a professional cyclist to the young riders who aspire to succeed in their careers. '' David will work with the squad on a voluntary basis until the end of the month with a view to subsequently joining the team in a more official capacity. \\\hline 
  Summary & British Cycling has revealed that David Millar, the former British road race champion who served a two-year doping ban, is mentoring its academy riders. \\\hline 
  Ours & Former Tour de France and Commonwealth gold medallist David Millar has joined British Cycling's anti-doping education team. \\\hline
  \makecell{Document\\(ID \#9858)} & The 22-year-old spent much of the 2015-16 season with the Blues, making 22 league appearances. Lloyd will not feature for Chester in Saturday's game at Maidstone as Jon McCarthy's side look for back-to-back victories in the National League. They beat Dagenham 3-0 on Tuesday, having lost their opening game by the same scoreline at Gateshead. Find all the latest football transfers on our dedicated page. \\ \hline
  Summary & National League club Chester have re-signed Port Vale midfielder Ryan Lloyd on loan until 1 January. \\ \hline
  Ours & National League side Chester have re-signed midfielder Jack Lloyd on a one-month loan deal from Championship side Fulham. \\ \hline
  
  \multicolumn{2}{c}{CNN DailyMail} \\ \hline
  \makecell{Document\\(ID \#3068)} & kilmarnock interim manager gary locke has been given the role on a permanent basis after signing a three-year deal. the former hearts boss joined the club as assistant boss to allan johnston last summer but took control of the team when his ex-tynecastle team-mate quit at the start of february. the 39-year-old - who will speak at a press conference on friday morning - has lost just once in seven games since taking over at rugby park. gary locke has been given the job at kilmarnock on a permanent basis after a successful interim spell . locke shakes hands with chairman jim mann after signing a three-year deal at the club . \\\hline
  Summary & gary locke has been interim manager since start of february . locke has won two and drawn four of his seven games in charge . the 37-year-old took over when allan johnston quit .\\\hline
  Ours & gary locke has been given the job at kilmarnock on a permanent basis . the former hearts boss joined the club as assistant to allan johnston last summer . locke has lost just once in seven games since taking over at rugby park. \\\hline
  \makecell{Document\\(ID \#4535)} & feeling sleepy at your desk? well, this docile dog could just sum up how you feel. shaheen pirouz from denton, texas, filmed her tiny pet canine being propped up and repeatedly falling forwards. footage shows him being positioned on his back legs, with his eyes immediately starting to close. he then flops over to one side as he falls into a deep sleep. pirouz is heard cooing in the background as she watches the sweet moment unfold. 'puppy had been awake for a few hours and couldn't help but fall asleep even in the funniest positions,' the filmer later wrote online. ready for bed: shaheen pirouz from denton, texas, filmed her tiny pet canine being propped up and repeatedly falling forwards . good night! footage shows him being positioned on his back legs, with his eyes immediately starting to close . \\\hline
  Summary & shaheen pirouz from denton, texas, filmed her tiny pet canine being propped up and repeatedly falling forwards . \\\hline
  Ours & shaheen pirouz from denton, texas, filmed her tiny pet canine being propped up and repeatedly falling forwards . \\\hline
  \makecell{Document\\(ID \# 5585)} & chelsea have suffered a blow in their pursuit of palermo's paulo dybala after the striker declared he 'would love to stay in serie a'. the 21 year old has scored 13 league this season and has also attracted interest from the likes of manchester united, arsenal, paris saint-germain and atletico madrid. but reports in italy suggest that juventus have offered 323million for dybala, who admitted he would love to play alongside andrea pirlo and does not 'speak a word of english or french'. palermo's paulo dybala has attracted interest from a number of leading clubs in europe . dybala (centre) has scored 13 league goals for palermo this season and could be on the move . 'i love italy. this is the country that made me famous and i would love to stay in serie a,' he said. 'there are some big teams out there who don't play in champions league and i can't deny that i'd love to play in europe's most prestigious competition. 'it's a lot easier for a striker when you have a playmaker like pirlo behind you,' he added. 'he makes even the most difficult things look easy.' \\\hline
  Summary & paulo dybala has attracted interest from a number of top european clubs . juventus favourites to sign striker after he says he wants to stay in italy . juventus have reportedly offered 323million to sign the chelsea target . click here to read all you need to know about dybala . \\\hline
  Ours & palermo striker paulo dybala has attracted interest from a number of clubs . reports in italy suggest juventus have offered 323million for the striker . dybala has scored 13 league goals for palermo this season . \\ \hline
  
  \multicolumn{2}{c}{NEWSROOM} \\ \hline
  \makecell{Document\\(ID \#304)} & This post is in partnership with Time. The article below was originally published at Time.com Apple users might want to think again if they havent already downloaded the iOS 8 upgrade. People have taken to Twitter and Apple forums to complain that their phones have been experiencing sluggish Wi-Fi and dwindling battery life, post-update. If this is proof of a genuine issue with the latest iteration of Apples operating system, it would be ironic considering that the update boasts features that identify apps that are the biggest battery sucks. Apple AAPL did not reply immediately for comment. But here are some disappointed Apple users airing their gripes on Twitter: @FintyWizard Ive been having some wifi issues with iOS 8. Have needed to power cycle the phone to get wifi back.  Luke Dickinson (@Dominitus) September 23, 2014 GAH. Is anyone else having problems with wifi dropping out with iOS 8? The unupdated iPad is fine, the iPhone is not.  boredjessica (@boredjessica) September 23, 2014 anyone experiencing problems with iOS 8, with slow app loading and poor battery life. Very frustrating :(  North Harrow No.6557 (@HarrowFreemason) September 23, 2014 So.... iOS 8 is a huge battery suck.  Tim White (@white\_tim) September 23, 2014 Anyone confused by iOS 8 can also read TIMEs tips and tricks guide to the new system. \\\hline
  Summary & Some iPhone and iPad users gripe about sluggish Wi-Fi and dwindling battery life post-update. \\\hline
  Ours & Some users are complaining about sluggish Wi-Fi and dwindling battery life. \\\hline
  
  
  
  \end{tabular}
  \caption{Generated summaries by $\text{PEGASUS}_{\text{LARGE}}$ (\gnews) on XSum, CNN DailyMail and NEWSROOM. The examples were randomly picked.}
  \label{tab:qualitative_1}
\end{table*}


\begin{table*}[h!]
\scriptsize
  \centering
  \renewcommand{\arraystretch}{1.3}
  \begin{tabular}{c|p{0.85\textwidth}}
  \hline
  \multicolumn{2}{c}{Multi-News} \\ \hline
  \makecell{Document\\(ID \#1045)} & LONDON (Reuters) - Prime Minister Theresa May survived a confidence vote from her Conservative party on Wednesday, but more than a third of her lawmakers said she was no longer the right leader to implement Britains exit from the European Union. Britain's Prime Minister Theresa May speaks at Prime Minister's Questions in the House of Commons, London, Britain, December 12, 2018. Parliament TV handout via REUTERS Britains March 29 exit has been plunged into crisis by parliamentary opposition to the divorce deal she struck with the EU last month, which has opened up possibilities including a delay to Brexit or even another referendum on membership. May on Monday cancelled a parliamentary vote on her Brexit deal, designed to maintain close future ties with the bloc and agreed after two years of negotiations, after it became clear she would lose it badly. Eurosceptic critics of the deal within her own party triggered a no-confidence vote in her leadership hours after she returned from talks with European leaders aimed at winning additional assurances about her deal. After two hours of voting in Committee Room 14 in the House of Commons, Graham Brady, chairman of the 1922 Committee of Conservative backbenchers, said 200 Conservative lawmakers had voted in support of May as leader, and 117 against, indicating her party was bitterly divided over the direction of Brexit. Supporters said the result showed the party should now get behind her. But the hardline Brexit supporters who triggered the vote because they saw her deal as a betrayal of the 2016 referendum said she should now quit. It is a terrible result for the prime minister, Jacob Rees-Mogg, leader of a hard Brexit faction in the party, told BBC Television. The prime minister must realise that, under all constitutional norms, she ought to go and see the queen urgently and resign. But May loyalist Chris Grayling, her transport minister, said the party had endorsed her comfortably. ENDANGERING BREXIT? May, who voted to remain in the EU in the 2016 referendum, had warned opponents of her withdrawal deal - struck after two years of negotiations - that if they toppled her, Brexit would be delayed or stopped. Shortly before the vote, May sought to win over wavering lawmakers by promising to step down before the 2022 election. Brexit is Britains most significant political and economic decision since World War Two. Pro-Europeans fear the departure will weaken the West as it grapples with the U.S. presidency of Donald Trump and growing assertiveness from Russia and China. The outcome will shape Britains \$2.8 trillion economy, have far-reaching \\\hline
  Summary & When Prime Minister Theresa May entered a room in the House of Commons to speak to Conservative lawmakers ahead of a no-confidence vote Wednesday, she was greeted by table banging customary sign of approval, reports the AP. It ended up being a prescient gesture: The BBC reports she needed the votes of 159 MPs to remain the Conservative leader, and she crossed that threshold, winning the confidence vote 200 votes to 117, reports the Guardian. It adds that after the words ``does have confidence in...'' were announced, it could not hear the rest due to the eruption of cheers. But Reuters reports May won't be in it for the long haul. In her pre-vote comments, she pledged to step down in advance of the 2022 parliamentary election. ``She did say she wouldn't be fighting the next general election,'' one minister was quoted as saying. ``It was quite emotional the way she put it, she said in my heart I wanted to do that but now I recognize that I am not going to.'' \\\hline
  Ours & British Prime Minister Theresa May survived a confidence vote from her Conservative party on Wednesday, but more than a third of her lawmakers said she was no longer the right leader to implement Britain's exit from the European Union. May on Monday canceled a parliamentary vote on her Brexit deal, designed to maintain close future ties with the bloc and agreed after two years of negotiations, after it became clear she would lose it badly. Eurosceptic critics of the deal within her own party triggered a no-confidence vote in her leadership hours after she returned from talks with European leaders aimed at winning additional assurances about her deal. After two hours of voting in Committee Room 14 in the House of Commons, Graham Brady, chairman of the 1922 Committee of Conservative backbenchers, said 200 Conservative lawmakers had voted in support of May as leader, and 117 against, indicating her party was bitterly divided over the direction of Brexit. Supporters said the result showed the party should now get behind her. But the hardline Brexit supporters who triggered the vote because they saw her deal as a betrayal of the 2016 referendum said she should now quit. ``It is a terrible result for the prime minister,'' Jacob Rees-Mogg, leader of a hard Brexit faction in the party, told BBC Television. ''The prime minister must realize \\\hline
  
  \multicolumn{2}{c}{Gigaword} \\ \hline
  \makecell{Document\\(ID \#4)} & at least \#\# people were killed as typhoon sepat hit the chinese mainland after more than \#\#\#,\#\#\# were evacuated as a precaution , state media reported . \\\hline
  Summary & storms lash chinese coast killing \#\# ; \#\#\#,\#\#\# evacuated as precaution \\\hline
  Ours & at least \#\# dead as typhoon sepat hits china \\\hline
  \makecell{Document\\(ID \#254)} & ministers from the european union and its mediterranean neighbors gathered here under heavy security on monday for an unprecedented conference on economic and political cooperation . \\\hline
  Summary & european mediterranean ministers gather for landmark conference by julie bradford \\\hline
  Ours & eu mediterranean ministers meet under heavy security \\\hline
  \makecell{Document\\(\# 998)} & chinese flights has logged more than five million continuous hours of safety , the longest such streak in the nation 's history . \\\hline
  Summary & china 's aviation industry sets safety flight record official \\\hline
  Ours & chinese flights record five million continuous hours of safety \\\hline
  
  \multicolumn{2}{c}{WikiHow} \\\hline
  \makecell{Document\\(ID \#4372)} & You can choose both winter shoes and summer shoes as your wardrobe evolves through the spring. Summer is the time to enjoy your sandals and espadrilles. Just be sure to enjoy them without socks. You can still be somewhat flexible as your wardrobe transitions to winter, but avoid the sandals and espadrilles. They don't match with the heavier fabrics and colors of autumn. Choose loafers, flats and boots. Make sure that your heels are wider to avoid slippage. \\\hline
  Summary & Be flexible in the spring. Lighten up in summer. Pull back in the fall. Choose practical shoes for winter. \\\hline
  Ours & Transition to summer shoes. Transition to winter shoes. \\\hline
  
  \multicolumn{2}{c}{Reddit TIFU} \\\hline
  \makecell{Document\\(ID \#967)} & this tifu happened just minutes ago, i'm writing through tears. for some background: i'm a senior in high school and for my graduation party, my parents are renovating our whole house. our hallways and doorways are abnormally skinny so we need to take apart everything if we want to move it to almost anywhere. i just moved into a new bedroom, so furniture is still working out the kinks since being put back together. onto the good stuff! i'm laying in bed watching netflix and decide that i am going to go to sleep after this episode. i make a move to get out of bed to turn off the lights, but there was a shift in my wooden bedframe. naturally, i pause, but since i'm in no apparent danger, i begin to climb out of bed. there's a relatively small gap between my mattress and the bedframe, and my left nut decided to take a field trip down there. at that same time, due to the lessened downward pressure, my bedframe settled again. suddenly good friends, the mattress and the bedframe become very close; unfortunately, i had the balls to try to keep them apart. with one testicle locked between the wrong wood and a surprisingly firm mattress, i trip, due to the unexpected resistance. i fall, land face-first, which yanks my nut free, and i immediately see stars. at first, i was confused. then, the first wave of pain hit and i knew i had screwed up, big. i have never felt as much pain as i have tonight. battling through manly eye-sweat, i eventually got to the light switch and crawled into bed. i guess i'll be sitting gingerly for a while. \\\hline
  Summary & got off my butt, almost busted a nut. \\\hline
  Ours & tried to climb out of bed, fell and broke my nut. \\\hline
  
  \end{tabular}
  \caption{Generated summaries by $\text{PEGASUS}_{\text{LARGE}}$ (\gnews) on Multi-News, Gigaword, WikiHow and Reddit TIFU. The examples were randomly picked.}
  \label{tab:qualitative_2}
\end{table*}




\begin{table*}[h!]
\scriptsize
  \centering
  \renewcommand{\arraystretch}{1.3}
  \begin{tabular}{c|p{0.85\textwidth}}
  \hline
  \multicolumn{2}{c}{BIGPATENT} \\ \hline
  \makecell{Document\\(ID \#1410)\\Truncated} &  the film school database will allow every student attending subscribed film schools the ability to become a member . each film school will potentially have a faculty admin account to add and modify certain items . lastly , there will be the global admin account , to manage all of the schools . the first version of the website runs on a linux based server using php , mysql and apache ( lamp ). additional storage for file uploads , and video files , and image uploads are stored on amazon s3 . the first version of the system uses a custom ffmpeg installation to encode uploaded videos for flash based playback . the first version of the system uses celltrust as the sms gateway to send sms messages through their api . after users have been granted access to the program , they will have the capability to create a personal profile , create projects , search for people and projects , send messages to other users , upload videos to their profiles and project profiles that they are associated with . guests ( non - users ) of filmschooldatabase . com will only have access to public pages , which will lack ( not have ) search functionality , profile / project creation / editing functionality , etc . public users must have the appropriate   public password   to be able to view the corresponding public user or project profile pages . cataloguing and linking is the main feature of the website . ... \\\hline
  Summary & the invention is an electronic networking system assisting college   film students   in the process of locating other film students as well as their fellow students ; film projects . the system includes features to search for projects and students within particular schools or throughout a plurality of schools . this system provides contact information and / or a means of contact , including an sms text messaging ability . \\\hline
  Ours & the present invention , film school database , is a unique computer database driven system and method for , storing , organizing , and sharing information related to film schools .\\\hline
  
  \multicolumn{2}{c}{arXiv} \\\hline
  \makecell{Document\\(ID \#1397)\\Truncated} & superconducting qubits are solid - state artificial atoms , comprising lithographically defined josephson tunnel junctions and superconducting interconnects . when cooled to milli - kelvin temperatures , these qubits exhibit quantized states of charge , flux , or junction phase depending on the circuit design parameters @xcite . associated with these quantized states is a spectrum of energy levels , tunable via an external control parameter , e.g. , an applied electric or magnetic field . although generally only the lowest two energy eigenstates are utilized for quantum information science applications , the energy spectrum indeed extends to higher - energy levels corresponding to higher - excited states of the circuit . the separation between pairs of energy levels typically falls in the radio frequency and microwave regimes , and resonantly driving the artificial atom with a harmonic field can couple and induce quantum - state transitions . due to their relatively large size , superconducting artificial atoms can be strongly coupled to their external control fields . it is this feature , along with their quantum coherence , that we utilize in the present article . a large - amplitude harmonic control field can drive an artificial atom throughout its energy - level spectrum . when driven through an avoided level crossing , a landau - zener - stckelberg ( lzs ) transition occurs . this is a coherent process akin to a beamsplitter for photons , taking an input state of the atom and outputting a superposition of states . ...\\\hline
  Summary & superconducting persistent - current qubits are quantum - coherent artificial atoms with multiple , tunable energy levels . in the presence of large - amplitude harmonic excitation , the qubit state can be driven through one or more of the constituent energy - level avoided crossings . the resulting landau - zener - stckelberg ( lzs ) transitions mediate a rich array of quantum - coherent phenomena . we review here three experimental works based on lzs transitions : mach - zehnder - type interferometry between repeated lzs transitions , microwave - induced cooling , and amplitude spectroscopy . these experiments exhibit a remarkable agreement with theory , and are extensible to other solid - state and atomic qubit modalities . we anticipate they will find application to qubit state - preparation and control methods for quantum information science and technology . \\\hline
  Ours & superconducting qubits are solid - state artificial atoms , comprising lithographically defined josephson tunnel junctions and superconducting interconnects . when cooled to milli - kelvin temperatures , their energy - level spectrum falls in the radio frequency and microwave regimes , and resonantly driving the artificial atom with a harmonic field can couple and induce quantum - state transitions . when driven through an avoided level crossing , a landau - zener - stckelberg ( lzs ) transition occurs . this is a coherent process akin to a beamsplitter for photons , taking an input state of the atom and outputting a superposition of states . repeated passages through an avoided crossing act as an atom interferometer , causing the atomic superposition state to interfere quantum mechanically with itself . we present three experimental works that utilize lzs transitions in a strongly - driven persistent - current qubit . the first is mach - zehnder - type interferometry between repeated lzs transitions , for which we observed quantum interference fringes in n - photon transition rates . the second is microwave - induced cooling , by which we achieved effective qubit temperatures less than 3 mk , a factor 10 - 100 times lower than the environmental temperature . the \\\hline
  
  \multicolumn{2}{c}{PubMed} \\\hline
  \makecell{Document\\(ID \#950)\\Truncated} & idiopathic generalized epilepsy ( ige ) is characterized by various combinations of generalized tonic clonic seizures , absence seizures , myoclonus ( blumenfeld , 2005 ; zhang et al . , 2011 ) , and generalized spike - and - wave discharges ( gswds ) observed during interictal periods on electroencephalography ( eeg ) recordings ( hamandi et al . , 2006 ; moeller et al . , 2011 ; zhang et al . , 2011 ) . focal spike wave complexes occasionally are observed interictally in patients with ige , although ictal eeg recordings show only generalized - onset seizures and no focal - onset seizures in ige ( drury and henry , 1993 ; seneviratne et al . , 2012 ) . unlike focal or partial epilepsy , which has a confined range of influence , ige affects the whole or a larger portion of the brain often without obvious , known cause ( engel , 2001 ) . among drug - resistant epilepsy , patients with focal epilepsy may receive surgical resection to become seizure free . on the other hand , patients with generalized epilepsy do not have such a treatment option . recently deep brain stimulation ( johnson et al . , 2013 ) has been hypothesized as a way to treat epilepsy patients ( fisher et al . , 2010 ) . ... \\\hline
  Summary & unlike focal or partial epilepsy , which has a confined range of influence , idiopathic generalized epilepsy ( ige ) often affects the whole or a larger portion of the brain without obvious , known cause . it is important to understand the underlying network which generates epileptic activity and through which epileptic activity propagates . the aim of the present study was to investigate the thalamocortical relationship using non - invasive imaging modalities in a group of ige patients . we specifically investigated the roles of the mediodorsal nuclei in the thalami and the medial frontal cortex in generating and spreading ige activities . we hypothesized that the connectivity between these two structures is key in understanding the generation and propagation of epileptic activity in brains affected by ige . using three imaging techniques of eeg , fmri and eeg - informed fmri , we identified important players in generation and propagation of generalized spike - and - wave discharges ( gswds ) . eeg - informed fmri suggested multiple regions including the medial frontal area near to the anterior cingulate cortex , mediodorsal nuclei of the thalamus , caudate nucleus among others that related to the gswds . the subsequent seed - based fm \\\hline
  Ours & there is general agreement that both cortex and thalamus participate in the generation of typical spike wave seizures , but their relative importance is still unclear . the goal of the present study is to use noninvasive , multimodal imaging techniques to elucidate the underlying mechanisms that generate generalized spike - and - wave discharges ( gswds ) in idiopathic generalized epilepsy ( ige ) patients . specifically , we aim to map the cortical networks associated with gswds and investigate the causality between cortex and thalamus during gswds . we first performed eeg - informed functional magnetic resonance imaging ( fmri ) analysis and identified regions of interest ( roi ) . we then tested the specific connectivity patterns by seed - based connectivity analysis in fmri data . the seeds include both regions determined by the eeg - informed fmri analysis and additional ones identified by eeg waveforms . the granger causality analysis to identify sources and sinks within the networks were further subjected to the granger causality analysis to identify sources and sinks within the networks . we found that the thalamus and cortex are involved in the generation of gswds in ige patients . \\\hline
  
  \end{tabular}
  \caption{Generated summaries by $\text{PEGASUS}_{\text{LARGE}}$ (\gnews) on BIGPATENT, arXiv and PubMed. The examples were randomly picked.}
  \label{tab:qualitative_3}
\end{table*}



\begin{table*}[h!]
\scriptsize
  \centering
  \renewcommand{\arraystretch}{1.3}
  \begin{tabular}{c|p{0.85\textwidth}}
  \hline
  \multicolumn{2}{c}{AESLC} \\ \hline
  \makecell{Document\\(ID \#1751)} & We are getting closer to finishing up the agreement to sale a license to use POPS and its source code to AEP. It looks like we agree in principal but I'm not comfortable with some of the language proposed by AEP. Since Barbara Gary is out until next Tuesday I don't anticipate us finishing up the agreement until the end of next week at the earliest. Given the timing we need to be able to turn around and deliver the application \& documentation by the end of November in order to receive all of the funds this year. I will be setting up a meeting with the application, DBA, DA and technical writing teams to make sure we are all on the same page and ready to deliver the application by the end of November. - Tommy \\\hline
  Summary & Status of the sale of POPS to AEP \\\hline
  Ours & POPS License - AEP \\\hline
  
  \multicolumn{2}{c}{BillSum} \\ \hline
  \makecell{Document\\(ID \#1248)\\Truncate} & SECTION 1. SHORT TITLE. This Act may be cited as the   Veterans Identity Protection Act'', or the   VIP Act''. SEC. 2. PURPOSES. The purposes of this Act are-- (1) to reimburse injured persons for injuries suffered as a result of the unauthorized use, disclosure, or dissemination of identifying information improperly released by or obtained from the Department of Veterans Affairs; and (2) to provide for the expeditious consideration and settlement of claims for those injuries. SEC. 3. DEFINITIONS. In this Act: (1) Director.--The term   Director'' means the Director of the Office of Veterans Identity Protection Claims. (2) Injured person.--The term   injured person'' means an individual-- (A) whose name or other personal identifying information is part of data of the Department of Veterans Affairs that-- (i) was stolen from the home of an employee of the Department of Veterans Affairs on or around May 3, 2006; (ii) was reported missing from the Birmingham VA Medical Center on or around January 22, 2007; or (iii) is otherwise compromised as a result of a security breach, including any action or ommission by an officer, employee, volunteer, or contractor (or employee of a contractor) of the Department of Veterans Affairs in contravention of any security policy or procedure of the Department that results in such a breach; and (B) who suffered an injury as a result of the unauthorized use, disclosure, or dissemination of personal identifying information that was included in data described in subparagraph (A). ...\\\hline
  Summary & Veterans Identity Protection Act or VIP Act - Establishes as an independent office in the executive branch the Office of Veterans Identity Protection Claims, headed by a Director, to receive, process, and pay claims for injuries suffered as a result of the unauthorized use, disclosure, or dissemination of identifying information stolen from the Department of Veterans Affairs (VA) or otherwise compromised as a result of a security breach. Authorizes judicial review of claim determinations. \\\hline
  Ours & Veterans Identity Protection Act - Establishes an independent office of the executive branch to receive, process, and pay claims in accordance with this Act, the Office of Veterans Identity Protection Claims. Requires the Director of such Office to investigate, consider, adjust, determine, grant, deny, or settle any claim for money damages asserted under this Act. Entitles an injured person to receive from the United States reimbursement for any injuries suffered as a result of the unauthorized use, disclosure, or dissemination of personal identifying information that was included in Department of Veterans Affairs (VA) data reported on or around May 3, 2006. Requires the Director to determine and fix the amount, if any, to be paid for one or more injuries suffered by the injured person in accordance with state law. \\\hline
  
  \end{tabular}
  \caption{Generated summaries by $\text{PEGASUS}_{\text{LARGE}}$ (\gnews) on AESLC and BillSum. The examples were randomly picked.}
  \label{tab:qualitative_4}
\end{table*}
